An SMDP Approach to Optimal PHY Configuration in Wireless Networks

In this work, we study the optimal configuration of the physical layer in wireless networks by means of Semi-Markov Decision Process (SMDP) modeling. In particular, assume the physical layer is characterized by a set of potential operating points, with each point corresponding to a rate and reliability pair; for example, these pairs might be obtained through a now-standard diversity-vs-multiplexing tradeoff characterization. Given the current network state (e.g., buffer occupancies), a Decision Maker (DM) needs to dynamically decide which operating point to use. The SMDP problem formulation allows us to choose from these pairs an optimal selection, which is expressed by a decision rule as a function of the number of awaiting packets in the source's finite queue, channel state, size of the packet to be transmitted. We derive a general solution which covers various model configurations, including packet size distributions and varying channels. For the specific case of exponential transmission time, we analytically prove the optimal policy has a threshold structure. Numerical results validate this finding, as well as depict muti-threshold policies for time varying channels such as the Gilber-Elliott channel.

==> intro5.tex <==

\section{Introduction}{\label{sec:intro}}

Recent advances in coding and modulation have allowed communication systems to approach the Shannon limit on a number of communication channels; that is, given the channel state (e.g. the signal-to-noise ratio of an additive white Gaussian noise - AWGN - channel), communication near the highest rate theoretically possible while maintaining low error probability is achievable.    However, in many communication systems, particularly wireless communication systems, the channel conditions which a given transmission will experience are unknown.  For example, consider the case of slow multipath fading without channel state information at the transmitter~\cite{tse_vishwanath}. Because of the uncertainty in the level of multipath fading, it is possible that the rate employed at the transmitter cannot be supported by the channel conditions, hence resulting in packet loss or ``outage''.  The outage capacity~\cite{tse_vishwanath}, which gives the rate for various outage probabilities, captures the tradeoff in such a situation.  If a low rate is employed, it is likely that the channel conditions will be such that transmission at that rate can be supported (low outage); if a higher rate is employed, the probability is higher that the channel conditions will be such that transmission at that rate cannot be supported (high outage).  In fact, a wide range of physical layers models can be addressed through such an approach, i.e., having asymmetric characterization of the operating points and their corresponding parameters.  Given this characterization, a crucial question is at which point to operate the physical layer given information available about the current state of the network.

Modern wireless networks are extremely dynamic, with channel parameters and traffic patterns changing frequently. Consequently, the key question addressed here is how can a sender \emph{dynamically decide} on the best physical layer strategy, given the channel and traffic parameters available to it, as well as its own status.   For example, consider a sender required to decide among the aforementioned physical layer strategies:  an approach incurring high packet loss yet a small transmission time, or one possibly having a lower packet loss but a larger transmission time. In this paper, we derive a framework for a Decision Maker (DM) wishing to maximize the system throughput by choosing the appropriate physical layer setting, while taking into account as many system parameters as possible, in this case, delay, packet losses and its current packet backlog status. The DM faces a choice of achieving increased success probability provided additional transmission time, and one would expect that this decision will be made with the queue status in mind, as a full queue causes new arrivals to be rejected, incurring potential throughput loss. Thus, our goal is to rigorously analyze this tension, and identify the optimal strategy.

The tradeoff between rate and reliability is a fundamental characteristic of the physical layer, and we are interested in this formulation largely because it captures much more than the simple point-to-point single-antenna communication used for illustration in the first paragraph above.   To provide a systematic method to consider how this characterization might be derived, consider the the now-standard diversity-multiplexing tradeoff approach originally applied to point-to-point multi-antenna systems~\cite{zheng_dym_tradeoff} but now extensively extended beyond that.  In particular, the diversity-multiplexing approach captures the fundamental tradeoff between rate (multiplexing) and reliability (diversity) for a number of interesting physical layer choices, including:  (1) point-to-point multiple-input and/or multiple-output (MIMO) systems \cite{zheng_dym_tradeoff}, where the transmitter can decide whether to send multiple streams (``multiplex'') from the multiple antennas or to send a single stream with redundancy (``diversity''), or a combination of the two; (2) half-duplex relay channels (e.g. \cite{karmakar2011diversity}), where the transmitter can decide to use the relay, or not, and how to allocate time to the transmit and receive functions of the half-duplex relay.  We are particularly interested in this latter example, and we will adopt terminology from a classical problem in relaying~\cite{laneman2004cooperative} to help clarify the competing options in succeeding sections.  However, we hasten to remind the reader that the results apply much more generally to the diversity-multiplexing protocol for any physical layer.

Our model is also relevant for sources transmitting packets of variable sizes. In particular, once the size of the leading packet in the buffer is known prior to the  the transmission,  selecting the point of the discussed tradeoff also selects the transmission time, which has a crucial impact on the future buffer occupancy. If the buffer is full and arriving packets are immediately rejected, the potential throughput associated with these packets is lost. Clearly, the decision rule and the tradeoff structure are not straightforward in such cases. Nonetheless, we consider them in our model.
\subsection{Main contribution}
Our main contributions are as follows.
%\begin{itemize}

\textbf{Problem formulation: } We formulate the problem of optimal dynamic PHY configuration for the transmitter with long-lived packets influx by a SMDP. The model is presented in generality, capturing finite buffer size, variable packet size, variable channel state, general transmission time distribution and a decision space which is associated with possible PHY configuration.

\textbf{Value function derivation: } We derive the equations for the value function of the SMDP in several interesting cases. These equations are obtained in a tractable form, allowing a solution by simple value iteration. 

\textbf{Threshold policy characterization: } When transmission times are exponentially distributed, we prove there exists an \emph{optimal policy with a threshold structure}; that is, the source should make use of the more reliable option if the number of pending packets is lower than a given threshold, and transmit with the higher rate option otherwise. We also show that the value function in this case is concave and increasing.

\textbf{Numerical investigation: } We explore different scenarios by simulations. In particular, we validate the threshold policy and concavity for the exponential case and observe similarity to this structure in other cases as well. In the case of a variable channel (e.g., the Gilbert-Elliott channel) we observe a \textit{multi-threshold} policy which is described by having a separate threshold for each channel mode.

%\end{itemize}	

While a preliminary paper \cite{s3paper} gave basic numerical results for a related model, to the best of our knowledge, this work is the first to \emph{analyze} this problem for a finite buffer at the source and generality of all other system parameters.

\vspace{-0.1in}

\subsection{Related work}


The pioneering works on the relay channel  date back to the seventies~\cite{elgamal}, when  
 T. Cover and E. Gamal posed the problem of determining the capacity region of the full-duplex relay channel.  Since then, there has been progress in determining the capacity region for    
the degraded case, as well as for several MIMO settings \cite{wang2005capacity} or a class of erasure channels~\cite{khalili}. Cooperative strategies and their performance in relay networks were considered in \cite{1499041}.   Nonetheless, in its full generality  the capacity region of the relay channel is   still unkown.    

% We start our related work list with the pioneering work of \cite{elgamal} on relay, which assumed full duplex channel. 

% Several interesting scenarios were solved since then, e.g., t %Yet, the problem in its most general form is still open. 
Works \cite{yeh2007throughput,urgaonkar2014delay} utilize maximum differential backlog (MDB) methods to stabilize queues thus achieving optimal throughput. In particular, 
Yeh and Berry \cite{yeh2007throughput} considered control policies for cooperative relay selection. The authors mainly concentrate on the transport level, hence do not capture physical level considerations e.g., fading environment and diversity increase.   %which account for queue dynamics in order to optimize both scheduling and routing.  
% in a network that contains  numerous relay nodes.
Our approach is different, as we combine the control on the packet (i.e. transport) level with PHY consideration, accounting for fading factors. The additional difference is that we assume control of a finite queue, hence inherently stable.


Recently, Urgaonkar and Neely~\cite{urgaonkar2014delay} considered a constrained resource allocation problem in a relay network under stringent delay constraints.   
The reliability versus delay trade-off in finite buffered networks was addressed in and  in wireless networks in \cite{altman2007constrained}. 

\cite{supittayapornpong2015achieving} proposes near-optimal throughput achieving algorithms for finite queues. 
Our work differs from such previous studies as we consider a different  approach to model the relay channel, namely semi-Markov decision processes (SMDP),  which allows us to analyze a broader set of both PHY and transport level settings and channels, to provide an optimal policy, for which we prove structural properties. % as opposed to those considered in~\cite{urgaonkar2014delay, supittayapornpong2015achieving, altman2007constrained}.


For a basic introduction to SMDPs we refer the reader to~\cite{puterman1994markov}. 
A number of previous works on SMDPs have focused on establishing the existence of optimal policies of  threshold type under a variety of settings~\cite{koole1998structural,hajek1984optimal,sennott2009stochastic,walrand1988introduction}.   To the best of our knowledge, none of these works have considered the optimality of  threshold policies for  SMDP models of  the relay channel.

%All these works can

%A large body of work is devoted to the scheduling perspective, assuming one or several relay nodes cannot receive and transmit simultaneously (half-duplex), and focusing on choosing the appropriate relays, optimal routing, etc. For example, Khojastepour \emph{et al.} \cite{aazhang} considered two \emph{modes} of operation in the context of `cheap' relays. Selection relaying schemes were considered in \cite{laneman2004cooperative} as a possible method to achieve cooperative diversity. 

The general trade-off between PHY rate and reliability has various important applications apart from the already mentioned basic relay channel. 
For example, the trade-off between multiplexing and diversity was discussed in~\cite{heath2002diversity} in the context of MIMO channels, in~\cite{tse2004diversity} in the context of multiple-access channel with fading, and in~\cite{liang2011cognitive} in the context of cognitive radio sensing techniques.

%A key feature, and a source for complications in such relay channels, is that they encompass both space and time diversity. That is, 
Space diversity can be achieved by transmitting simultaneously through two channels, minimizing the effects of fading in a single slot, while time diversity can be achieved since fading also varies over time, hence different schemes can be used at different times. Works  such as
Berry and Gallager~\cite{gallager} and
Collins and Cruz~\cite{cruz} accounted for time diversity and delay constraints, while works such as Scaglione, Goeckel and Laneman~\cite{goeckel} accounted for space diversity.  The SMDP framework introduced in this paper  accounts for both space and time diversity.  

\vspace{-0.1in}




==> mdp_model4.tex <==
\vspace*{-5pt}\section{SMDP-based formulation and solution} \label{sec:mdpmodel}
%In this section, we define the general form of the SMDP and give specific examples.
Denote SMDP with average cost functional by tuple \sdo{\{\bS,\bA,\bP,r\}}, where the components stand for the state space, the action space, the transition probabilities and the reward function. 
We consider the most general case where the state \sdo{s\in\bS} is expressed by the triplet
$(n,h,k)\in\R^3$ where $n$ stands for the number of information chunks in the system, $h$ stands for the medium (channels) state and $k$ stands for the size of the packet (measured in number of chunks) which is to be transmitted in the upcoming transmission.  The state transitions happen after transmission over either possible path (``a" or ``b") ends, or, in the case there was no ready packet for the transmission (e.g. the buffer was empty), the chunk which just has arrived indicates that the only packet awaiting now in the queue is ready. We assume that a \textit{transmission mode} (i.e. transmission decision) with corresponding parameters (e.i. corresponding transmission rates) to each transmission path is attributed. Right after the state transition the decision which sets the  transmission mode of the current packet is made, and its transmission is immediately started.


% For simplicity, whenever it is relevant, we will assume henceforth that the buffer maximal capacity is given by $B+1$.
% Observe that due to the structure of the model described above, the state which corresponds to having the maximal number of chunks, $B+1$ is not defined.
%We present Bellman equations which see states right after accomplished transmissions. 
%Hence,,  At this point of time, we have to account for all possible transitions. This includes number of arrivals, channel transitions and leading packet size transitions. 
%To this end, we specify the state structure. 

%direct and relay transmission times for different packet size, and the time it takes till the first packet arrival to the queue.
%Therefore, we assume packet size transition probabilities, denoted by $q_i(k'|k)$ depend on the action $i$, $\i\in\{r,d\}$. %Denote  $q_i(A|A)$, $q_i(B|A)$, $q_i(A|B)$, $q_i(B|B)$, where $i\in\{d,r,0\}$ is the action.
% The size of the second and the third dimension of the state is specified according to the physical parameters
The probability of having $j$ chunks after transmission interval of length $t$ is denoted by \rdo{\varrho(j|i,t)} and is governed by a Poisson distribution with mean \sdo{\lambda t}, e.g. if $j<B+1$,$i>0$ then $j=i-k+m$, where $m$ is the number of arrivals during time $t$. 
%(\textbf{TODO} - or 2nd+3rd can be seen as additional single dimension)
%However, they can depend on the action attempted in the same slot.
The action space is defined by $\bA=\{a,b,0\}$, standing for transmission mode "a", transmission mode "b", and abstaining from transmission. In the case the buffer was empty or action $0$ was selected, no transmission is initiated, while the next decision will be performed right after the next packet is ready. Otherwise, the actions are taken right after the accomplished transmissions.
%The number of arrivals between two consecutive departures is given by Poisson distribution.
%Note that if the source is not empty, a packet is transmitted immediately after the preceding transmission end. 
The instantaneous gain at the end of a successful transmission is given by $r=k$, in the case the reward is set according to the packet size, and $r=1$ in the case successfully transmitted packets of all sizes have the same value.


\begin{comment}
Write the general cost function associated with initial state $s_0$ and policy \rdo{\pi\in\calU}, where \rdo{\calU} is the set of all admissible policies (i.e. non-anticipating and always acting such that~\eqref{eq:100} is not violated), as follows 
\reqs{0}{J(s_0)=\E\sum_{n=0}^\infty\int_{\sigma_{n}}^{\sigma_{n+1}} e^{-\gamma t} r_ndt}
Note that %$s_n$ is the state at which decision epoch $n$ was made and
$\sigma_n$ is the time at which decision epoch $n$ occurred yielding reward $r_n$. For notational convenience, we assume  $\sigma_0=0$.
\end{comment}
%\sbe
% J(t)=\E\sum_{n=0}^\infty\int_{\sigma_{n}}^{\sigma_{n+1}} e^{-\gamma s} r_ndt
%\see
%where $r_n$ denotes reward for transmission $n$, %$R(s)$ is Poisson counting process which mean will be specified below.
 %when the initial state $s_0$ is given.
%Due to the stationary property we will assume the initial time $t=0$, and will omit the time mark where it is clear.
In order to simplify the forthcoming analysis, we use a discounted infinite horizon SMDP defined by tuple \sdo{\{\bS,\bA,\bP,r,\gamma\}}, where the first four components are exactly the same as in the average cost formulation and $\gamma$ is a discount factor. The discounted cost is given by the following
%\small
\begin{comment}
\req{-5}
{J^\pi(s_0)=\E\sum_{m=0}^\infty e^{-\gamma\sigma_{m}} r_m =\E r^\pi(s_0)+\E\sum_{m=1}^\infty e^{-\gamma\sigma_{m}} r_m}
{eq:disc}
\normalsize
\end{comment}
\begin{align}
J^\pi(s_0)&=\E\sum_{m=0}^\infty e^{-\gamma\sigma_{m}} r_m =\E r^\pi(s_0)+\E\sum_{m=1}^\infty e^{-\gamma\sigma_{m}} r_m = \nonumber \\
& =\E r^\pi(s_0)+J^{\pi,1}(s_0)  \label{eq:disc}
\end{align}
The connection between discounted criterion and average infinite reward criterion is well understood. 
In particular, under mild conditions for $\gamma$, they possess the \textit{similar optimal policy}, which is named the Blackwell optimal policy. See~\cite{bertsekas1995dynamic} for the details. 
Note that the second term of~\eqref{eq:disc} is a result of applying dynamic programming and it is given by \sdo{\E_{(\sigma_1,s_1)}[ e^{-\gamma\sigma_1}V(s_1)]}.
The superscript $\pi$ stands for the policy and the value function is given by $V(s_0)=\max_\pi J^\pi(s_0)$, for all $s_0\in\bS$.
%For cost, which treats the general state formulation can be expressed as follows. \sdo{s_0=\{i,h,k\}} and \sdo{s_1=\{j,h',k'\}} write
%In order to simplify the analysis, we assume that the reward for the transmission is accumulated at the \textit{beginning} of the transmission. As long as the time distribution of the upcoming transition is known, we weigh that reward by the corresponding average discount at the end of the transmission.
We now expand for all possible transitions. 
Denote the transition probability $P(s_1|s_0,\pi(s_0))$. Accounting for number of arrivals, channel transitions and leading packet size transitions, for $s_0=(h,k,i)$,  write
\begin{align}
& P(s_1|s_0,\pi(s_0))=P((h',k',j)|(h,k,i),\pi(s_0)) = \nonumber\\
& = q^{\pi(s_0)}(k'|k)p^{\pi(s_0)}(h'|h)\varrho(j|i,t)
\end{align}
The Bellman equation is given by~\eqref{eq:disc}, setting ${J}^{\pi,1}(s_0) $ as follows
\begin{align}
&{J}^{\pi,1}(s_0) = \\
&=\sum_{s_1=(h',k',j)}V(s_1) \int_0^\iy e^{-\gamma t}P(s_1|s_0,\pi(s_0))g^{\pi(s_0)}(t)dt\label{eq:be1}\\
&=\sum_{h'}\sum_{k'}\sum_{j=i-k}^{B-k+1}V(s_1)\int_0^\iy e^{-\gamma t}P(s_1|s_0,\pi(s_0))g^{\pi(s_0)}(t)dt.\label{eq:be2}
\end{align}
%
\begin{comment}
\iflong\else\footnotesize\fi
\ral{-5}{
& J^\pi(s_0)= \E r^\pi(s_0)+\Big[\sum_{s_1=(h',k',j)}V(s_1)\cdot\nonumber\\
&\int_0^\iy e^{-\gamma t}P(s_1|s_0,\pi(s_0))g^{\pi(s_0)}(t)dt\Big]=\label{eq:be1}\\
&\E r^\pi(s_0)+ \Big[\sum_{h'}\sum_{k'}\sum_{j=i-k}^{B-k+1}V(s_1)\cdot\nonumber\\
&\int_0^\iy e^{-\gamma t}P(s_1|s_0,\pi(s_0))g^{\pi(s_0)}(t)dt\Big].\label{eq:be2}}
\iflong\else\normalsize\fi
%\end{equation}}}
\end{comment}
%
%
% $\E r^\pi(s_0)$ is the expected average reward at the initial state $s_0$. 
The first (i.e the outer) summation in~\eqref{eq:be2} is over all possible next channel states.
 It is degenerated if the channel is fixed. The second summation is over all possible packet sizes to be transmitted at state $s_1$. If packet size is unknown, or all packet sizes are equal, this sum degenerates. The third summation is over the number of arrivals to the queue during the first transmission. The integration accounts for the average time the first transmission interval takes. Hence, the transmission time pdf $g^{\pi(s_0)}$ may depend on the action taken in state $s_0$. 
The expected reward at state $s_0$ is added up at the \textit{end of the transmission} and is calculated by
\(\E r^\pi(s_0)=\int r^{\pi(s_0)}e^{-\gamma t}g^{\pi(s_0)}(t)dt\). Note that $r^0=0$, while $r^a=k(1-p_a),\;r^b=k(1-p_b)$. Also note that in the case $i<k$, (i.e. the first and the only packet in the buffer is still waiting for remaining chunks to arrive) the $g^{\pi(s_0)}(t)$ is given by distribution time of remaining $k-i$ packets to arrive and the reward is zero. 
\iflong Observe that each product of probabilities of the form $q^{\pi(s_0)}(k'|k)p^{\pi(s_0)}(h'|h)\varrho(j|i,t)$ is a weight of the corresponding value function at the next state $s_1$. \fi
The optimal value function is retrieved by the maximization over all admissible policies 
${V(s_0)=\max_\pi J^\pi(s_0)}$. 
%\small
%\reqs{-10}{V(s_0)=\max_\pi J^\pi(s_0)}
%\normalsize

\begin{comment}
For the Poisson arrivals at the finite buffered queue with capacity $\BS$ it is given by
\sdo{P(i|j,t)=\frac{e^{-\mu t}(\mu t)^{i-j+1}}{(i-j+1)!}}, \sdo{P(i|0,t)=\frac{e^{-\mu t}(\mu t)^{i}}{(i)!}}, \sdo{P(B|j,t)=\sum_{i=B}^\iy\frac{e^{-\mu t}(\mu t)^{i-j+1}}{(i-j+1)!}}
%\label{be2}
Not that $1$ is subtracted since the decision epochs are at the ends of transmissions.
\end{comment}
We bring next \iflong three \else two \fi examples, for which the corresponding Bellman equations can be written in the tractable form and the value functions can be explicitly calculated, e.g. by value iteration~\cite{puterman1994markov}. \iflong
Note that for all examples the boundary conditions at buffer limits are separately written.
\else

Note that for all Bellman equations at buffer limits boundary conditions are separately written. We omitted here these details. 
\fi
\iflong
\input{exp_SMDP1}
\fi
\input{det_fixed2}
\input{uniform2}







==> mdp_model_O.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace*{-5pt}\section{SMDP-based formulation and solution} \label{sec:mdpmodel}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this paper we utilize a semi-Markov decision process (SMDP) which is widely used in modeling stochastic control problems. SMDPs are characterized by a set of states, a set of actions associated with each such state, a transition probability for a given action and a reward function associated with the action result, where the sojourn time spent in a particular state follows an arbitrary probability.


Next, we introduce the SMDP formulation for the optimal PHY configuration problem.  We start with definition of the state-space. A state ${s\in\bS}$ is expressed by the triplet $(n,h,k)\in\R^3$, capturing  the number of packets present in the system including the one being transmitted ($n$), the medium (channels) state ($h$) and the size of the packet which is to be transmitted in the upcoming transmission ($k$).

Transmissions can take one of two possible configurations (``a" or ``b"). Correspondingly, the action space is given by $\bA=\{a,b\}$, standing for transmission modes ``a" and ``b", respectively. We assume that a \textit{transmission mode} (i.e., transmission decision) with corresponding parameters (i.e., corresponding transmission rates) is attributed at every decision epoch.

%\newline

The SMDP follows the evolution of the system at decision points. Accordingly, state transitions occur after either service completions or a packet arrival to an empty system. Obviously a decision regarding the next packet transmission mode after a service completion is made only if the system is not empty. If after a service completion the queue is left empty, the decision is postponed until the next packet arrival.


%\newline

The state transition probabilities are governed by the number of new arrivals during the time elapsed between the two consecutive state. For example, the probability of having $j$ packets in the buffer after transmission of a packet, given that the packet transmission elapsed $t$ time units and the buffer initially contained $i$ packets, is denoted by \rdo{\varrho(j|i,t)} and is governed by a Poisson distribution with mean ${\lambda t}$.  Specifically, if $j<B+1$ and $i>0$ then $\varrho(j|i,t)=\frac{(\lambda t)^{j-i-1}}{n!}e^{-\lambda t }$. The rest of the state transition probabilities can be computed in the same straightforward manner. Note that the time $t$ elapsed between the two consecutive states, which is the packet transmission time, depends on the packet size and on the action (configuration) taken by the DM (obviously if the buffer is left empty, the time until the next transition is distributed according to exponential distribution and in the next state the buffer contains exactly one packet).

Let $\{ \sigma_m\}$, $m=0,1,\ldots$,  be a time series where $\sigma_m$ is the instant at which the $m$-th reward is added. Positive rewards are accumulated at the end of successful service completions.  Let $r_m$ be a random variable characterizing the $m$th reward. Then, $r_m > 0$  when $\sigma_m$ corresponds to completion of a successful service; otherwise, $r_m = 0$.
Let us rewrite the discounted cost given in (\ref{Eq_AverageDiscountedReward}), conditioning on the first event (transition). Accordingly, the average discounted reward comprises the sum of the reward obtained at the first state transition and the average discounted residual throughput profit associated with future rewards. Specifically:

%
\begin{align}
& J^\pi(s_0) =\E r^\pi(s_0)e^{-\gamma\sigma_{0}}+\E\sum_{m=1}^\infty e^{-\gamma\sigma_{m}} r_m  \nonumber \\
& =\E r^\pi(s_0)+J^{\pi}_1(s_0)  \label{eq:disc}
\end{align}% \end{align}

Note that the second term of~\eqref{eq:disc} is given by ${\E_{(\sigma_1,s_1)}[ e^{-\gamma\sigma_1}V(s_1)]}$, where $s_1$ is the state following $s_0$. The superscript $\pi$ stands for the policy under consideration. Further note that the value function $V$ is obtained by maximizing $J$ over all feasible policies, and is given by $V(s_0)=\max_\pi J^\pi(s_0)$, for all $s_0\in\bS$.

Denote the transition probability from state $s_0=(h,k,i)$ to state $s_1=(h',k',j)$ by $P(s_1|s_0,\pi(s_0),t)$. $P(s_1|s_0,\pi(s_0),t)$ depends on the  arrival process, channel dynamics and leading packet size, and is given by
\begin{align}
& P(s_1|s_0,\pi(s_0),t)=P((h',k',j)|(h,k,i),\pi(s_0),t) = \nonumber\\
& = q(k'|k)p(h'|h)\varrho(j|i,t)
\end{align}
where $\sum_{k',h',j}q(k'|k)p(h'|h)\varrho(j|i,t)=1$.

The Bellman equation for the initial state $s_0$, action $\pi(s_0)$ and  next state $s_1$ is given by~\eqref{eq:disc}, setting ${J}^{\pi}_1(s_0) $ as follows
\begin{align}
&{J}^{\pi}_1(s_0) = \E e^{-\gamma t}\sum_{s_1}V(s_1)P(s_1|s_0,\pi(s_0)=u_0,t)\label{eq:be0}\\
&=\sum_{s_1}V(s_1) \int_0^\iy e^{-\gamma t}P(s_1|s_0,u_0)g^{u_0}(t)dt\label{eq:be1}\\
&=\sum_{h'}\sum_{k'}\sum_{j=i-k}^{B-k+1}V(s_1)\int_0^\iy e^{-\gamma t}P(s_1|s_0,u_0)g^{u_0}(t)dt.\label{eq:be2}
\end{align}
The first (i.e the outer) summation in~\eqref{eq:be2} is over all possible next channel states. It is degenerated if the channel state is fixed. The second summation is over all possible packet sizes to be transmitted at state $s_1$. This sum degenerates if the packet size is unknown at decision time, or when all packet sizes are equal. The third summation is over the number of arrivals to the queue during a transmission. The integration accounts for the transmission time. Note that the transmission time pdf $g^{\pi(s_0)}$ may depend on the action taken in state $s_0$.
 The expected instantaneous reward at state $s_0$ accounts for the average discount at the end of the transmission:
\begin{equation}
\E r^\pi(s_0)=\int r^{\pi(s_0)}e^{-\gamma t}g^{\pi(s_0)}(t)dt,\label{eq:8}
\end{equation}
where $\pi(s_0) \in \{a,b\}$, $r^{a}=k(1-p_a)$ and $r^{b}=k(1-p_b)$.

The tractability of the Bellman equation form depends on resolvability of the integration in~\Crefrange{eq:be0}{eq:be2}. In the case where a closed form can be obtained, a convenient utilization of value iteration (see, e.g., ~\cite{puterman1994markov}) procedure is possible. In particular,~\Crefrange{eq:be0}{eq:be2} substituted in~\eqref{eq:disc} results in recursive equations. Then, the repetitious application of~\eqref{eq:disc} guarantees that convergence of $V$ to the fixed point which is the unique solution can be an arbitrary closed.



%\ifArx
\subsubsection{Chunk granularity}\label{subsubsec1}
In order to consider packets composed of variable number of chunks, several technical adjustments should be made. In particular, the Poisson \textit{chunk arrival process} would feed the buffer room, which should be measured in \textit{chunk units}. The packet size can be indicated within the last or the first chunk in a packet (i.e, in correspondence with the two modes of packet size impact on the decision making).
%In order to incorporate a general definition of having packets larger than one chunk,
The state definition should include the number of chunks in the buffer, hence,~\Crefrange{eq:be0}{eq:be2} should be accordingly adjusted to reflect the change in the queue size after each transmission. In addition, the calculation of~\eqref{eq:8} should account for all additional states where the number of chunks present in the buffer is less than one packet.
%\ifArx
%In particular, if the head-of-line packet  is incomplete we have  $i<k$, the instantaneous reward is zero  and $g^{\pi(s_0)}(t)$ is the pdf of the  remaining time  for the missing $k-i$ chunks to arrive.
%\fi
%\fi
%\iflong Each product of the form $q(k'|k)p(h'|h)\varrho(j|i,t)$ can be interpreted as a weight of the  value function at the next state $s_1$, where $\sum_{k',h',j}q(k'|k)p(h'|h)\varrho(j|i,t)=1$. \fi
%The optimal value function is retrieved by the maximization over all admissible policies
%${V(s_0)=\max_\pi J^\pi(s_0)}$.
%\small
%\reqs{-10}{V(s_0)=\max_\pi J^\pi(s_0)}
%\normalsize
% Observe that~\eqref{eq:be2} depends on the integration result, where the integrand is a product of two probability density functions and exponential discount.

%Hence, the tractability of the final equation depends on resolvability of the integration. In the case a closed form can be obtained, a convenient utilization of value iteration (see, e.g., ~\cite{puterman1994markov}) procedure is possible. This would allow arbitrary close convergence of $V$ to the fixed point which is the unique solution. In particular, by repetitious application of the recursive~\Crefrange{eq:exp2}{eq:exp1},  $V$ converges to the unique solution.
\begin{comment}
For the Poisson arrivals at the finite buffered queue with capacity $\BS$ it is given by
\sdo{P(i|j,t)=\frac{e^{-\mu t}(\mu t)^{i-j+1}}{(i-j+1)!}}, \sdo{P(i|0,t)=\frac{e^{-\mu t}(\mu t)^{i}}{(i)!}}, \sdo{P(B|j,t)=\sum_{i=B}^\iy\frac{e^{-\mu t}(\mu t)^{i-j+1}}{(i-j+1)!}}
%\label{be2}
Not that $1$ is subtracted since the decision epochs are at the ends of transmissions.
\end{comment}


% We bring next \iflong three \else two \fi examples, for which the corresponding Bellman equations can be written in the tractable form. %and the value functions can be explicitly calculated, e.g. by value iteration~\cite{puterman1994markov}.
%\iflong
%Note that for all examples the boundary conditions at buffer limits are separately written.
%\else

%Note that for all Bellman equations at buffer limits boundary conditions are separately written. We omitted here these details.
%\fi
\iflong
\input{exp_SMDP1}
\fi
\input{det_fixed2}
\input{uniform2}







==> phy_model4.tex <==
\begin{figure}
	\center
	\includegraphics[scale=0.29]{3to2}
	\vspace*{-5pt}\caption{Relay channel logical model}\label{fig:32} \vspace*{-15pt}
\end{figure}

\section{System model and metrics}{\label{sec:phy}}
We assume the application level at the source (S) produces packets to be transmitted to the destination (D). %The packets 
The structure of packets is discussed in sequel.
The source attempts to communicate the packet at the head of the queue, formed in a \textit{finite sized buffer}, to the destination by a choice among the possible operating points of the physical layer. In the case there is an ongoing transmission of an earlier produced packet, the new packets are fed into the queue, space permitting. The packets arriving at full buffer are rejected and the retransmission details are taken care of by the application level. For presentation and analytical simplicity, we assume a pair of operating points at all decision epochs.  While this choice applies cleanly to the simple half-duplex relay channel example, the extension to the situation of more than two possible operating points, as might be appropriate for other PHY layer architectures, is straightforward.
Also note that in the case of continuous intervals of operating points, the model can be addressed by known techniques for continuous action space, e.g., discretization.
The tension is clear: a higher rate choice that uses less resources (time) but at a higher packet loss probability, or a lower rate choice that exploits more resources to obtain a lower packet loss probability.


\subsubsection*{\textbf{Transmission modes}} 
We assume two possible operating points, and we use a nomenclature motivated by the application of the diversity-multiplexing tradeoff to a classic half-duplex relay channel choice: the more reliable and lower relaying rate and outage probability from a prototypical early cooperative diversity protocol, and the less reliable and higher rate corresponding to the direct choice. 
In all scenarios mentioned in this paper, we will always denote the more reliable path with a lower rate as path ``a", while the less reliable path with a higher rate  will be denoted as path ``b". Denote the rates $R_a$ and $R_b$, where $R_a<R_b$. The corresponding packet losses are denoted as $p_a$ and $p_b$, where $p_a<p_b$ at all times.
%relaying (``r") choice, with rate $R_r$
%with rate $R_d$ and outage $p_d$. 

%{\bf DG:  Not sure I quite understand "For convenience, we will refer to the relay transmission time as an atomic period." in the new context. MSh: let's use the clarification in blue instead? }  
We consider packets of random length, hence, the rates of the two options yield transmission time probability density functions $g^{b}(t)$ and $g^{a}(t)$, which are readily calculated from the packet length distribution, $R_a$ and $R_b$. Note that in the case of a half duplex relay model $g^{a}(t)$ refers to the entire path associated with choice ``a", even if the latter is subdivided into two separate paths. Therefore, we aim to analyze a simplified configuration as Figure~\ref{fig:32} demonstrates. 
Note that the upper illustration particularly fits the relay channel problem, while the lower one can also refer to the general tension between two PHY settings associated with two different propagation paths; the upper path corresponds to the choice of reliability (diversity) while the lower path corresponds to the choice of rate (multiplexing). 
\subsubsection*{\textbf{Variable channel}} 
We assume that a variable channel can be modeled by a Markov process; that is, the \textit{current channel statistics} are independent of the past given the last state of the channel. These dynamics reflect well-known channel models (e.g., i.i.d. fading, Gilbert-Elliot model).   
Consider a sequence of fading values observed across source packets, each value corresponding to a channel (or, separately, to each path) state.  
We assume that the statistics are known to the DM and are constant for a period which is significantly longer than the longest possible packet transmission time. Hence the DM can obtain the packet losses associated with each such fading value for each potential PHY configuration.
Note that we allow generality of these probabilities by assuming they can be different for different transmission modes. Clearly, \rdo{\sum_{h'}p^u(h'|h)=1}. 
\iflong Also, for the empty buffer state, we allow these probabilities to be distinct from those at other buffer states, hence capturing the time it takes until the first packet arrival to the queue. \fi 
While these assumptions are approximations, they conform to the well-known realistic slow fading model, or quasi-static channels. Denote the channel state by $h$, and the channel transition probability from state $h$ to state $h'$ by $p^u(h'|h)$, where the superscript $u$, $u\in\{a,b\}$ denotes the transmission mode. %($r$: relay; $d$: direct). 
 %Also note that in the case of high variance of transmission times, the compliance with the channel dynamics model can be easily achieved by careful tuning of channel transition probabilities defined above.

\subsubsection*{\textbf{Arrival process}} We assume that the \textit{chunks} arrival process at the source is a Poisson process with intensity $\lambda$. The size of the buffer is known to the DM and is given by $B$ chunks. The packet is ready to be transmitted once the newly arrived chunk indicates that it is the last one in the packet.
%Once the buffer is full, the application instantly stops producing new chunks till new room is available. Hence, the buffer overflow can be interpreted as a potential loss of successful transmissions. 
Therefore, this model captures the following packet sizing options:
\begin{enumerate}
\item Each packet can have a size of one or more chunks. After each transmission, the corresponding number of chunks is subtracted from the buffer.
\item The packets of all sizes occupy space of exactly one chunk. (For example, packet descriptors are stored in the buffer, or the chunks are large enough to fit the maximal possible packet size.) After each transmission, exactly one chunk is subtracted from the buffer.
\end{enumerate} 
%We assume  While this assumption merely simplifies notation and relaxes some technical details, the analytical model can be easily extended in order to reflect packet sizes which can occupy variable number of slots.
%Let $B$ be the buffer capacity % and  $n \in \{0,1,\ldots,B-1\}$ be the number of chunks currently stored in the waiting   line 
%(maximum number of packets
%in the system, including the packet being transmitted).
%(not counting the chunk currently under transmission). %Denote the size of the packet at the head of the source's queue (in the case it can be sampled prior to the transmission and thus be part of the \textit{state} thus having impact on the decision) by $k$. 
We allow \textit{two modes} of packet size impact. In the first mode, the packet size is unknown prior to the transmission, and the transmission times are merely distributed with $g^u$ defined above. Note that this can model the scenario where application produces chunks and starts the transmission before the last chunk of the packet has been produced. In the second mode, the size can be sampled prior to the transmission. Then, the size of the packet to be transmitted is a part of the \textit{state} and has impact on the decision. Denote the size of the packet in this case by $k$.
%Hence, in the case the packet size is known, it will determine the transmission time. Otherwise, the transmission time is given by a corresponding probability density function (pdf), denoted by \rdo{g^u(t)}.
Then, \textit{packet size transition probabilities}, denoted by $q^u(k'|k)$, stand for the probability of 
having packet of size $k'$ at the head of the line after transmitting packet of size $k$ by acting $u$, where $u\in\{a,b\}$.
\iflong And, as in the case of the channel transition probabilities, these probabilities can be different for the empty buffer state to allow for the possibility of a different size distribution for the first packet to arrive into the empty buffer. \fi  
We assume a finite set of possible packet sizes such that \rdo{\sum_{k'}q^u(k'|k)=1} for each possible action $u$. Hence, in the first mode, $g^u$ can be merely assumed as deterministic given the packet sizes, or be independent of packet size and selected from other system parameters.  
Note that $q^u$ can capture complex packet arrival patterns. %, rather than mere Poisson process. 
For example, a sequence of big packets which is likely to be followed by sequence of small patterns and vice versa can be modeled provided the appropriate values for $q^u$ are selected. We assume that the packet arrival process and variable channel process are independent.
%With the coding rate $r_t$ information bits per channel symbol fixed throughout this work, the variable packet length is worked into our model by mapping it to a variable transmission time, which, because of the extra time involved for relaying, depends on the path $r$ or $d$ selected \iflong\footnote{Note that for a physical layer operating at capacity, (\ref{m1}) is valid regardless of the packet length.}\else    (Note that for a physical layer operating at capacity, (\ref{m1}) is valid regardless of the packet length.)\fi.
 %Clearly, this pdf can capture the distribution of the packet size; however, our general model makes no assumptions about \rdo{g^u(t)}, and hence it can return any positive values and capture other model aspects, if desired.
%Naturally, this distribution depends on action (i.e. the transmission path) to be attempted by the source.
%We will refer to this time as an atomic period for both relay and direct paths. 

%Before the start of each new transmission the source observes the number of packets awaiting in the queue, and, possibly, the channel state and the size of the packet to be transmitted.  Per above, the source has a characterization of the channel fading processes and thus, conditioned on its knowledge (e.g. prior channel state) the packet loss probability on each of the two paths is readily obtained.  %The performance criterion is related to the successful transmission of packets, as follows.  Denote the starting time of transmission slot $m$, where $m\in\{0,1,\cdots\}$ by $\sigma_m$. Assume $\sigma_0=0$. 
%Each transmission slot a reward $r_m$ is obtained.  

\subsubsection*{\textbf{General performance criterion} }
We now define the performance criterion, which will suit our SMDP formulation as defined in the next section.
%\iflong
%The performance criterion is the expected total discounted infinite horizon reward which is given by the following well-known definition %\iflong
%
%\rals{-5}{
%J=&\E\int_0^\infty e^{-\gamma t} r(t)dt=\E\sum_{m=0}^\infty\int_{\sigma_{m}}^{\sigma_{m+1}} e^{-\gamma t} r_mdA(t)}	%\fi
%
%where $\gamma$ is a discount factor and $r(t)$ is a reward accumulated at time $t$. The equality is reasoned by the fact that in our model rewards are only awarded at discrete time points (e.g. transmission opportunities ends) denoted by $\sigma_m$, $m\in\{0,1,\cdots\}$ that is, where the differential of counting process $A$, counting the transmission attempts and formally defined by 
%\[A(t)=\sup\{l\geq0:\sum_{i=0}^l\tau_i<t\},\] where $\tau_i=\sigma_i-\sigma_{i-1}$, is positive. However, in general, the reward function $r(t)$ allows to capture continuous cost, e.g. energy cost which can be proportional to the buffer occupancy at time $t$. Note that $r_m$ may be equivalent to a size of the successfully decoded packet transmitted in transmission opportunity $m$, or to a constant reward $r_m=C$, regardless of its size; it may incorporate additional cost factors predefined by DM. Without loss of generality, we assume that lost or dropped packets yield no reward. 
%\else
%The performance criterion is the expected total discounted infinite horizon reward which is given by the following well-known definition %\iflong
Denote the ending time of $m$-th transmission attempt as $\sigma_m$, $m\in\{0,1,\cdots\}$. We assume that the rewards are only added up at transmission ending times. Hence, in the case the transmission at time $\sigma_m$ was successful, the reward worth of $r_m$ was positive. Otherwise, $r_m$ was equal to zero. %Hence, average reward for action $u$ is given by $C(1-p_u)$. 
Define average reward over infinite horizon
%In this paper, we only allow lump rewards at ending times of successful transmission attempts, denoted by $\sigma_m$, $m\in\{0,1,\cdots\}$.  We assumed a constant reward $r_m=C$, regardless of a packet size, however our model covers any lump reward function.

\rals{-10}{
%J=&\E\int_0^\infty e^{-\gamma t} r(t)dt=\E\sum_{m=0}^\infty e^{-\gamma\sigma_m} r_m}	%\fi
J^A=&\lim_{N\to\infty}\frac{1}{N}\E\sum_{m=1}^N  r_m} %=\E\sum_{m=0}^\infty e^{-\gamma\sigma_m} r_m}
\iflong\else\normalsize\fi
%where $\gamma$ is a discount factor and $r(t)$ is a reward accumulated at time $t$.  %it may incorporate additional cost factors predefined by DM. Without loss of generality, we assume that lost or dropped packets yield no reward. 
%\fi%\iflong The second inequality merely solves the integral.\fi %Note that the expected value is over the interval boundaries as. 
Thus, our goal is the following:

Find the \textit{dynamic physical layer setting selection policy}, which takes as input the current occupancy of the buffer and information (if any) on the current state of the channel and the packet size at the source's queue head, and provide as an output a decision on which transmission path to employ, such that $J^A$ is maximized.  \iflong 

We formulate the described problem by a Semi Markov Decision Process (SMDP), as formally defined in the next section.\fi
\iflong
\begin{table}[t]
\center
\begin{tabular}{l|l}
\hline
variable & description \\
\hline
% $\bS$ & state space of SMDP  \\
% $\bA$ & action space \\
% $\calU $ & policy space  \\
                $\lambda$ & arrival rate \\
$\BS$ & buffer capacity (maximum number of packets \\
& in the system, including the packet being transmitted) \\\hdashline
% $N$ & random variable characterizing number  of packets in  & $N \in \{0,1,\ldots,B-1 \}$  \\
% & queue, i.e.,  waiting queue + under transmission & \\ 
%             & (as states are tracked  right after  a service & \\ 
%          &   completes, $N \leq B-1$) & \\   
$s$ & SMDP state (buffer state and channel state) \\
& Note: as state transitions occur after departures, the buffer \\
 & state after a transition  ranges between 0 and $B-1$ \\      
   $V(s)$ &   value function at state $s$, $V(s)=\max\{V^{(r)}(s),V^{(d)}(s)\}$ \\
    $V^{(u)}(s)$ &   cost associated with decision $u$ at state $s$, $u \in \{ a,b\}$   \\
  %   $V^{(b)}(s)$ &  cost associated with decision ``b" at state $s$     \\   \hdashline
    %$c_r$ & instantaneous relay throughput (reward) & $(1-p_r)C\beta_r$ \\
     %   $c_d$ & instantaneous direct throughput (reward) & $(1-p_d)C\beta_d$ \\
        $\beta_{u,s}$ &  discount associated with action $u$ \\
        $k$ &  number of frames  per packet \\
                     $\tau_{u,s}$ & mean time to transmit via channel $u$ at state $s$ \\
       %  $\tau_{b,s}$ & mean time to transmit via channel ``b" at state $s$ \\
                $\mu_{u,s}$ & transmission rate of channel $u$,          $\tau_{u,s} = 1/\mu_{u,s}$ \\ \hdashline
       % $\mu_{b,s}$ & transmission rate of channel ``b",           $\tau_{b,s} = % 1/\mu_{b,s}$ \\ \hdashline
        $p_u$ & packet loss probability associated with channel $u$, $u \in \{a,b\}$ \\ 
  %      $p_b$ & packet loss probability associated with channel ``b"\\   \hdashline
%        $\gamma$ & discount factor \\ 
%        $\pi$ & policy (subscript) \\ \hdashline
        $g^{\pi}(t)$ & pdf of transmission time then using policy $\pi$ \\ 
        $P^u(j|i,t)$ & probability of $j-i$ arrivals after $t$ time units, given a \\
        & buffer initially filled with $i$ packets and action  $u$  is taken  \\
        $p^u(h'|h)$ & channel transition probabilities, given  action $u$ is taken \\
        $q^u(k'|k)$ & packet size transition probabilities, given  action  $u$ is taken \\
       \hline
\end{tabular}
\vspace{-2pt}
\caption{SMDP notation.} \vspace{-0.3in} %\label{tab:general}
\end{table}
\fi

==> phy_model55.tex <==
\begin{figure}
	\center
	\includegraphics[scale=0.29]{3to2}
	\vspace*{-5pt}\caption{Relay channel logical model}\label{fig:32} \vspace*{-15pt}
\end{figure}

\section{System model and metrics}{\label{sec:phy}}
The system is defined according to the following set of assumptions.
\subsubsection*{\textbf{Arrival process}} 
We assume the application layer at the source (S) produces packets to be transmitted to the destination (D). 
% We assume that the \textit{chunks arrival process} at the source is a Poisson process with intensity $\lambda$. 
Packets are produced by the application  according to a Poisson process with rate $\lambda$ and feed a \emph{finite buffer}.     

The buffer is divided into $B$ slots, and each packet consumes one slot.   % with capacity $B$.      
  Packets, in turn, are divided into chunks, and the transmission time of a packet  depends  on its size.  
  We consider two alternative models to capture such a dependency, varying according to the amount of information available to the decision maker at decision time.     In both cases, we assume that  packet sizes are %independent and identically distributed, 
  drawn from a known distribution.  
  Under  the first model, however, we assume that  the samples drawn  are unknown prior to decision making, whereas under the second model we assume that the size of the packet to be transmitted is  part of the \textit{state} and has an impact on the decision process. % Denote the size of a packet in this case by $k$..   
   
   
%    cannot be timely sampled by the DM before transmission, hence is unknown prior to the transmission. Then, transmission times are random as it specified in sequel. 
%  In the second mode, the size can be sampled prior to the transmission. Then, the size of the packet to be transmitted is a part of the \textit{state} and has impact on the decision. Denote the size of a packet in this case by $k$.
%Hence, in the case the packet size is known, it will determine the transmission time. Otherwise, the transmission time is given by a corresponding probability density function (pdf), denoted by \rdo{g^u(t)}.


Next, we characterize the   dynamics of packet sizes.  
Let $q(k'|k)$ be the  \textit{packet size transition probability}, i.e.,  the probability of 
having packet of size $k'$ at the head of the line (HOL) after transmitting packet of size $k$. % by acting $u$, where $u\in\{a,b\}$.
%\iflong And, as in the case of the channel transition probabilities, these probabilities can be different for the empty buffer state to allow for the possibility of a different size distribution for the first packet to arrive into the empty buffer. \fi  
We assume a finite set of possible packet sizes such that \rdo{\sum_{k'}q(k'|k)=1}. %for each possible action $u$. 
%
% DANIEL: I REMOVED THIS SENTENCE AS I DID NOT UNDERSTAND IT ence, in the first mode, the transmission time can be both merely assumed as a deterministic function of a given packet size, or to be independent of a packet size and selected from other system parameters.  
%
Note that $q$ can capture complex packet arrival patterns. %, rather than mere Poisson process. 
For example, a sequence of big packets which is likely to be followed by sequence of small packets and vice versa can be modeled provided the appropriate values for $q$ are selected. 
%Also note that in the case of continuous intervals of operating points, the model can be addressed by known techniques for continuous action space, e.g., discretization.

  
  The source attempts to transmit the  HOL packet %, formed in a \textit{finite sized buffer}, 
 to the destination, selecting one  among the possible \textit{operating points} offered by the physical layer.    
  While being transmitted, a packet must remain in the buffer.  After a service completion, exactly one packet is removed from the buffer.   
  Packets produced by the source when the buffer is  full are discarded.  
  
  %Retransmissions   may be executed at  the application level, and studying their impact is out of the scope of this work. 

  
%
% While our model allows to incorporate a general definition of having packets larger than one chunk,
% for the model simplicity, it is assumed packets of all sizes occupy space of exactly one chunk. (For example, packet descriptors are stored, or the chunks are large enough to fit the maximal possible packet size.) %Nevertheless, we assume that the packet sizes 
% With slight abuse of terminology, will use the term packet in sequel.


% The size of the buffer is known to the DM and is given by $B$ packets.  After each transmission, exactly one packet is subtracted from the buffer.
%The packets 
%The structure of packets is discussed in sequel.
%In the case there is an ongoing transmission of an earlier produced packet, the new packets are fed into the queue, space permitting. 


% Regardless of the space occupied by packets (or descriptors), the transmission time is allowed to depend on the actual packet size. 
\begin{comment}Note that this can model the scenario where application produces chunks and starts the transmission before the last chunk of the packet has been produced. 
\end{comment}


\subsubsection*{\textbf{Channel dynamics}} 
We assume that channel state dynamics can be modeled by a Markov process; that is, the \textit{current channel statistics} are independent of the past given the last state of the channel. These dynamics reflect well-known channel models (e.g., i.i.d. fading, Gilbert-Elliot model). 
Denote the channel state by $h$, and the channel transition probability from state $h$ to state $h'$ by $p(h'|h)$. %, where the superscript $u$, $u\in\{a,b\}$ denotes the transmission mode. 
Clearly, \rdo{\sum_{h'}p(h'|h)=1}.  
Next, consider a sequence of fading values observed across source packets, each value corresponding to a channel (or, separately, to each path) state.  
We assume that the statistics are known to the DM and are constant for a period which is significantly longer than the longest possible packet transmission time, hence independent of transmission mode. Hence the DM can obtain the packet loss probabilities associated with each such fading value for each potential PHY configuration.
%Note that we allow generality of these probabilities by assuming they can be different for different transmission modes.  
%\iflong Also, for the empty buffer state, we allow these probabilities to be distinct from those at other buffer states, hence capturing the time it takes until the first packet arrival to the queue. \fi 
While these assumptions are approximations, they conform to the well-known realistic slow fading model, or quasi-static channels.

\subsubsection*{\textbf{Transmission modes}} 
For presentation and analytical simplicity, we assume at most two possible operating points at all decision epochs. To exemplify this particular scenario, consider a simple half-duplex relay channel. Namely, we are motivated by the application of the diversity-multiplexing tradeoff to a classic half-duplex relay channel choice: the more reliable and lower relaying rate and outage probability from a prototypical early cooperative diversity protocol, and the less reliable and higher rate corresponding to the direct choice.
While this choice applies cleanly to this simple example, the extension to the situation of more than two possible operating points, as might be appropriate for other PHY layer architectures, is straightforward.
Henceforth, in all scenarios mentioned in this paper, a nomenclature of half-duplex relay channel will be used. We will always denote the more reliable path with a lower rate as path ``a", while the less reliable path with a higher rate  will be denoted as path ``b". Denote the rates $R_a$ and $R_b$, where $R_a<R_b$. The corresponding packet loss probabilities are denoted as $p_a$ and $p_b$, where $p_a<p_b$ at all times.
The reader should note that the limitation to only two operating points rules out the option of abstaining from a transmission. While the latter case opens an additional interesting tradeoff in certain cases (e.g., opting to wait for better channel conditions when the buffer is not full) we omit it here for the sake of simplicity of presentation. Yet, the straightforward extension to include the option of not to transmit for the certain time period is technically tractable; the interested reader is referred to the on-line version of the paper for the details.
%relaying (``r") choice, with rate $R_r$
%with rate $R_d$ and outage $p_d$. 

%{\bf DG:  Not sure I quite understand "For convenience, we will refer to the relay transmission time as an atomic period." in the new context. MSh: let's use the clarification in blue instead? }  
%We consider packets of random length, hence, 

The rates associated with the two operating points yield transmission time probability density functions (pdf) $g^{b}(t)$ and $g^{a}(t)$, which are readily calculated $R_a$ and $R_b$ and, possibly, from the size of the packet to be transmitted. Note that in the case of a half duplex relay model $g^{a}(t)$ refers to the entire path associated with choice ``a", even if the latter is subdivided into two separate paths. Therefore, the example of a half duplex relay obtains a simplified configuration, as Figure~\ref{fig:32} demonstrates. 
See that the upper illustration particularly fits the relay channel problem, while the lower one can also refer to the general tension between two PHY settings associated with two different propagation paths; the upper path corresponds to the choice of reliability (diversity) while the lower path corresponds to the choice of rate (multiplexing). 

 

  %($r$: relay; $d$: direct). 
 %Also note that in the case of high variance of transmission times, the compliance with the channel dynamics model can be easily achieved by careful tuning of channel transition probabilities defined above.
%Once the buffer is full, the application instantly stops producing new chunks till new room is available. Hence, the buffer overflow can be interpreted as a potential loss of successful transmissions. 
%Therefore, this model captures the following packet sizing options:
\begin{comment}
\begin{enumerate}
\item Each packet can have a size of one or more chunks. After each transmission, the corresponding number of chunks is subtracted from the queue in the buffer.
\item The packets of all sizes occupy space of exactly one chunk. (For example, packet descriptors are stored in the buffer, or the chunks are large enough to fit the maximal possible packet size.) After each transmission, exactly one chunk is subtracted from the buffer.
\end{enumerate} 
\end{comment}




To finalize, the tension is clearly understood: a higher transmission rate choice that uses less resources (time) but at a higher packet loss probability, or a lower transmission rate choice that exploits more resources to obtain a lower packet loss probability.

\subsubsection*{\textbf{General performance criterion} }
We now define the performance criterion. %, which will suit our SMDP formulation as defined in the next section.
%\iflong
%The performance criterion is the expected total discounted infinite horizon reward which is given by the following well-known definition %\iflong
%
%\rals{-5}{
%J=&\E\int_0^\infty e^{-\gamma t} r(t)dt=\E\sum_{m=0}^\infty\int_{\sigma_{m}}^{\sigma_{m+1}} e^{-\gamma t} r_mdA(t)}	%\fi
%
%where $\gamma$ is a discount factor and $r(t)$ is a reward accumulated at time $t$. The equality is reasoned by the fact that in our model rewards are only awarded at discrete time points (e.g. transmission opportunities ends) denoted by $\sigma_m$, $m\in\{0,1,\cdots\}$ that is, where the differential of counting process $A$, counting the transmission attempts and formally defined by 
%\[A(t)=\sup\{l\geq0:\sum_{i=0}^l\tau_i<t\},\] where $\tau_i=\sigma_i-\sigma_{i-1}$, is positive. However, in general, the reward function $r(t)$ allows to capture continuous cost, e.g. energy cost which can be proportional to the buffer occupancy at time $t$. Note that $r_m$ may be equivalent to a size of the successfully decoded packet transmitted in transmission opportunity $m$, or to a constant reward $r_m=C$, regardless of its size; it may incorporate additional cost factors predefined by DM. Without loss of generality, we assume that lost or dropped packets yield no reward. 
%\else
%The performance criterion is the expected total discounted infinite horizon reward which is given by the following well-known definition %\iflong
Consider an SMDP with discounted cost functional, characterized  by the tuple \sdo{\{\bS,\bA,\bP,r, \gamma\}}, where the components stand for the state space, the action space, the transition probabilities, the reward function and  the discount factor. The state space expresses the set of all possible combinations of buffer state, channel state, and leading packet size. The action space is a set of actions which fits exactly one action to one operating point. The state transitions probability space is calculated according to the transmission, arrival times distribution and channel and packet size dynamics. The reward is a symbolic representation of the accumulated throughput and, finally,  $\gamma$ is an appropriately selected constant.

Denote the ending time of $m$-th transmission attempt as $\sigma_m$, $m\in\{0,1,\cdots\}$. Clearly, positive rewards can be only added up at $\sigma_m$. The rewards, $r_m$ are r.v's, with expected value calculated in correspondence with some given policy $\pi$. Namely, in the case the transmission at time $\sigma_m$, according to selected action is successful, the reward was positive. In all other cases, $r_m$ is equal to zero.
Define $J^\pi(s_0)=\E\sum_{m=0}^\infty e^{-\gamma\sigma_{m}} r_m$.
In order to apply the dynamic programming principle, we view the states right after the transmission starts. Define the augmented time series $\eta_m$, $m\in\{0,1,\cdots\}$, such that in the case the transmission is initiated at a non-empty system, the average discounted reward given by $\E r_me^{-\gamma\eta_{m}}$ is awarded. Hence, in the case the transmission starts right after arrival to the empty buffer, $r_m=0$, at $\eta_m$.

Write the discounted cost as the sum of reward obtained for the first transmission and average discounted residual throughput profit associated with future rewards. 
%
%\small
\begin{comment}
\req{-5}
{J^\pi(s_0)=\E\sum_{m=0}^\infty e^{-\gamma\sigma_{m}} r_m =\E r_0^\pi(s_0)+\E\sum_{m=1}^\infty e^{-\gamma\sigma_{m}} r_m}
{eq:disc}
\normalsize
\end{comment}
\begin{align}
& J^\pi(s_0) =\E r^\pi(s_0)e^{-\gamma\eta_{0}}+\E\sum_{m=1}^\infty e^{-\gamma\eta_{m}} r_m  \nonumber \\
& =\E r^\pi(s_0)+J^{\pi}_1(s_0)  \label{eq:disc}
\end{align}% \end{align}

Thus, our goal is the following: find the \textit{dynamic physical layer setting selection policy $\pi$}, which takes as input the current occupancy of the buffer and information (if any) on the current state of the channel and the packet size at the source's queue head, and provide as an output a decision on which transmission path to employ, such that $J^\pi(s_0)$ is maximized.  

Note that the analysis that follows can be easily extended to account for an average cost criteria, defined by 
 $J^A=\lim_{N\to\infty}\frac{1}{N}\E\sum_{m=1}^N  r_m$ in the sense that both criteria possess  \textit{similar optimal policies}. 
The connection between discounted and average infinite reward criteria is understood via Blackwell optimality as it is demonstrated in e.g.,~\cite{bertsekas1995dynamic}.
%In particular, under mild conditions on $\gamma$, they  referred to as Blackwell optimal~\cite{bertsekas1995dynamic}.

 %Hence, average reward for action $u$ is given by $C(1-p_u)$. 
%Define average reward over infinite horizon
%In this paper, we only allow lump rewards at ending times of successful transmission attempts, denoted by $\sigma_m$, $m\in\{0,1,\cdots\}$.  We assumed a constant reward $r_m=C$, regardless of a packet size, however our model covers any lump reward function.

%\rals{-9}{
%J=&\E\int_0^\infty e^{-\gamma t} r(t)dt=\E\sum_{m=0}^\infty e^{-\gamma\sigma_m} r_m}	%\fi
%J^A=&\lim_{N\to\infty}\frac{1}{N}\E\sum_{m=1}^N  r_m} %=\E\sum_{m=0}^\infty e^{-\gamma\sigma_m} r_m}
%\iflong\else\normalsize\fi
%where $\gamma$ is a discount factor and $r(t)$ is a reward accumulated at time $t$.  %it may incorporate additional cost factors predefined by DM. Without loss of generality, we assume that lost or dropped packets yield no reward. 
%\fi%\iflong The second inequality merely solves the integral.\fi %Note that the expected value is over the interval boundaries as. 


Hence, we formulate the described problem by a discounted SMDP, which is formally explained in the next section.


\begin{table}[h!]
\center
\begin{tabular}{l|l}
\hline
variable & description \\
\hline
% $\bS$ & state space of SMDP  \\
% $\bA$ & action space \\
% $\calU $ & policy space  \\
                $\lambda$ & arrival rate \\
$\BS$ & buffer capacity (including the packet being transmitted) \\\hdashline
% $N$ & random variable characterizing number  of packets in  & $N \in \{0,1,\ldots,B-1 \}$  \\
% & queue, i.e.,  waiting queue + under transmission & \\ 
%             & (as states are tracked  right after  a service & \\ 
%          &   completes, $N \leq B-1$) & \\   
$s$ & SMDP state (buffer state,channel state,leading packet size) \\
%& Note: as state transitions occur after departures, the buffer \\
% & state after a transition  ranges between 0 and $B-1$ \\      
   $V(s)$ &   value function at state $s$, $V(s)=\max\{V^{(r)}(s),V^{(d)}(s)\}$ \\
    $V^{(u)}(s)$ &   cost associated with decision $u$ at state $s$, $u \in \{ a,b\}$   \\
  %   $V^{(b)}(s)$ &  cost associated with decision ``b" at state $s$     \\   \hdashline
    %$c_r$ & instantaneous relay throughput (reward) & $(1-p_r)C\beta_r$ \\
     %   $c_d$ & instantaneous direct throughput (reward) & $(1-p_d)C\beta_d$ \\
        $\beta_{u,s}$ &  discount associated with action $u$ \\
        $k$ &  number of frames  per packet \\
                     $\tau_{u,s}$ & mean time to transmit via channel $u$ at state $s$ \\
       %  $\tau_{b,s}$ & mean time to transmit via channel ``b" at state $s$ \\
                $\mu_{u,s}$ & transmission rate of channel $u$,          $\tau_{u,s} = 1/\mu_{u,s}$ \\ \hdashline
       % $\mu_{b,s}$ & transmission rate of channel ``b",           $\tau_{b,s} = % 1/\mu_{b,s}$ \\ \hdashline
        $p_u$ & packet loss probability associated with channel $u$, $u \in \{a,b\}$ \\ 
  %      $p_b$ & packet loss probability associated with channel ``b"\\   \hdashline
%        $\gamma$ & discount factor \\ 
%        $\pi$ & policy (subscript) \\ \hdashline
        $g^{\pi}(t)$ & pdf of transmission time when using policy $\pi$ \\ 
        $P^u(j|i,t)$ & probability of $j-i$ arrivals after $t$ time units, given a \\
        & buffer initially filled with $i$ packets and action  $u$  is taken  \\
        $p(h'|h)$ & channel transition probabilities \\
        $q(k'|k)$ & packet size transition probabilities\\%, given  action  $u$ is taken \\
       \hline
\end{tabular}
\vspace{-2pt}
\caption{SMDP notation.} \vspace{-0.25in} %\label{tab:general}
\end{table}


==> phy_model6.tex <==
\begin{figure}
	\center
	\includegraphics[scale=0.29]{3to2}
	\vspace*{-5pt}\caption{Relay channel logical model}\label{fig:32} \vspace*{-15pt}
\end{figure}

\section{System model and metrics}{\label{sec:phy}}
The system is defined according to the following set of assumptions.
\subsubsection*{\textbf{Arrival process}} 
We assume the application level at the source (S) produces data to be transmitted to the destination (D). 
We assume that the \textit{packets arrival process} at the source is a Poisson process with intensity $\lambda$. 
We consider packet sizes can vary, yet,
for the model simplicity, it is assumed packets of all sizes occupy space of exactly one slot of a \textit{finite sized buffer}. (For example, consider the case where packet descriptors are stored). The straightforward extension to consider packets occupying in the buffer a varying number of \textit{chunks}  is addressed in~\ref{subsubsec1}. 
The size of the buffer is known to the DM and is given by $B$ packets. The packets arriving at full buffer are rejected and the retransmission details are taken care of by the application level.
%Nevertheless, we assume that the packet sizes 
%With slight abuse of terminology, will use the term packet in sequel.
The source attempts to communicate the packet at the head of the queue to the destination by a choice among the possible \textit{operating points} of the physical layer.
 %The packets 
%The structure of packets is discussed in sequel.
%In the case there is an ongoing transmission of an earlier produced packet, the new packets are fed into the queue, space permitting. 
 

The transmission time is allowed to depend on the actual packet size. We consider \textit{two modes} to capture such a dependency. In the first mode, the packet size cannot be timely sampled by the DM, hence is unknown prior to the transmission. Then, transmission times are random as it is specified in sequel. 
\begin{comment}Note that this can model the scenario where application produces chunks and starts the transmission before the last chunk of the packet has been produced. 
\end{comment}
In the second mode, the size can be sampled prior to the transmission. Then, the size of the packet to be transmitted is a part of the \textit{state} and has impact on the decision. Denote the size of a packet in this case by $k$.
%Hence, in the case the packet size is known, it will determine the transmission time. Otherwise, the transmission time is given by a corresponding probability density function (pdf), denoted by \rdo{g^u(t)}.
Then, \textit{packet size transition probabilities}, denoted by $q(k'|k)$, stand for the probability of 
having packet of size $k'$ at the head of the queue after transmitting packet of size $k$. % by acting $u$, where $u\in\{a,b\}$.
%\iflong And, as in the case of the channel transition probabilities, these probabilities can be different for the empty buffer state to allow for the possibility of a different size distribution for the first packet to arrive into the empty buffer. \fi  
We assume a finite set of possible packet sizes such that \rdo{\sum_{k'}q(k'|k)=1}. %for each possible action $u$. 
Hence, the transmission time distribution can depend both on the size of a packet to be transmitted and on the other parameters which impact the system state.  
Note that $q$ can capture complex packet arrival patterns. %, rather than mere Poisson process. 
For example, a sequence of big packets which is likely to be followed by sequence of small packets and vice versa can be modeled provided the appropriate values for $q$ are selected. 
%Also note that in the case of continuous intervals of operating points, the model can be addressed by known techniques for continuous action space, e.g., discretization.


\subsubsection*{\textbf{Channel dynamics}} 
We assume that channel state dynamics can be modeled by a Markov process; that is, the \textit{current channel statistics} are independent of the past given the last state of the channel. These dynamics reflect well-known channel models (e.g., i.i.d. fading, Gilbert-Elliot model). 
Denote the channel state by $h$, and the channel transition probability from state $h$ to state $h'$ by $p(h'|h)$. %, where the superscript $u$, $u\in\{a,b\}$ denotes the transmission mode. 
Clearly, \rdo{\sum_{h'}p(h'|h)=1}.  
Next, consider a sequence of fading values observed across source packets, each value corresponding to a channel (or, separately, to each path) state.  
We assume that the statistics are known to the DM and are constant for a period which is significantly longer than the longest possible packet transmission time, hence independent of transmission mode. Hence the DM can obtain the packet loss probabilities associated with each such fading value for each potential PHY configuration.
%Note that we allow generality of these probabilities by assuming they can be different for different transmission modes.  
%\iflong Also, for the empty buffer state, we allow these probabilities to be distinct from those at other buffer states, hence capturing the time it takes until the first packet arrival to the queue. \fi 
While these assumptions are approximations, they conform to the well-known realistic slow fading model, or quasi-static channels.

\subsubsection*{\textbf{Transmission modes}} 
For presentation and analytical simplicity, we assume at most two possible operating points at all decision epochs. To exemplify this particular scenario, consider a simple half-duplex relay channel. Namely, we are motivated by the application of the diversity-multiplexing tradeoff to a classic half-duplex relay channel choice: the more reliable and lower relaying rate and outage probability from a prototypical early cooperative diversity protocol, and the less reliable and higher rate corresponding to the direct choice.
While this choice applies cleanly to this simple example, the extension to the situation of more than two possible operating points, as might be appropriate for other PHY layer architectures, is straightforward.
Henceforth, in all scenarios mentioned in this paper, a nomenclature of half-duplex relay channel will be used. We will always denote the more reliable path with a lower rate as path ``a", while the less reliable path with a higher rate  will be denoted as path ``b". Denote the rates $R_a$ and $R_b$, where $R_a<R_b$. The corresponding packet loss probabilities are denoted as $p_a$ and $p_b$, where $p_a<p_b$ at all times.
The reader should note that the limitation to only two operating points out-rules the option of abstaining from a transmission. While the latter case opens an additional interesting tradeoff in certain cases (e.g., Gilbert-Elliot channel,~\cite{altman2007constrained,s3paper}), we omit it here for the sake of simplicity of presentation. Yet, the straightforward extension to include the option of not to transmit for the certain time period is technically tractable; the interested reader is referred to the on-line version of the paper for the details.
%relaying (``r") choice, with rate $R_r$
%with rate $R_d$ and outage $p_d$. 

%{\bf DG:  Not sure I quite understand "For convenience, we will refer to the relay transmission time as an atomic period." in the new context. MSh: let's use the clarification in blue instead? }  
%We consider packets of random length, hence, 

The rates associated with the two operating points yield transmission time probability density functions (pdf) $g^{b}(t)$ and $g^{a}(t)$, which are readily calculated $R_a$ and $R_b$ and, possibly, from the size of the packet to be transmitted. Note that in the case of a half duplex relay model $g^{a}(t)$ refers to the entire path associated with choice ``a", even if the latter is subdivided into two separate paths. Therefore, the example of a half duplex relay obtains a simplified configuration, as Figure~\ref{fig:32} demonstrates. 
See that the upper illustration particularly fits the relay channel problem, while the lower one can also refer to the general tension between two PHY settings associated with two different propagation paths; the upper path corresponds to the choice of reliability (diversity) while the lower path corresponds to the choice of rate (multiplexing). 

 

  %($r$: relay; $d$: direct). 
 %Also note that in the case of high variance of transmission times, the compliance with the channel dynamics model can be easily achieved by careful tuning of channel transition probabilities defined above.
%Once the buffer is full, the application instantly stops producing new chunks till new room is available. Hence, the buffer overflow can be interpreted as a potential loss of successful transmissions. 
%Therefore, this model captures the following packet sizing options:
\begin{comment}
\begin{enumerate}
\item Each packet can have a size of one or more chunks. After each transmission, the corresponding number of chunks is subtracted from the queue in the buffer.
\item The packets of all sizes occupy space of exactly one chunk. (For example, packet descriptors are stored in the buffer, or the chunks are large enough to fit the maximal possible packet size.) After each transmission, exactly one chunk is subtracted from the buffer.
\end{enumerate} 
\end{comment}




To finalize, the tension is clearly understood: a higher transmission rate choice that uses less resources (time) but at a higher packet loss probability, or a lower transmission rate choice that exploits more resources to obtain a lower packet loss probability.

\subsubsection*{\textbf{General performance criterion} }
We now define the performance criterion. %, which will suit our SMDP formulation as defined in the next section.
%\iflong
%The performance criterion is the expected total discounted infinite horizon reward which is given by the following well-known definition %\iflong
%
%\rals{-5}{
%J=&\E\int_0^\infty e^{-\gamma t} r(t)dt=\E\sum_{m=0}^\infty\int_{\sigma_{m}}^{\sigma_{m+1}} e^{-\gamma t} r_mdA(t)}	%\fi
%
%where $\gamma$ is a discount factor and $r(t)$ is a reward accumulated at time $t$. The equality is reasoned by the fact that in our model rewards are only awarded at discrete time points (e.g. transmission opportunities ends) denoted by $\sigma_m$, $m\in\{0,1,\cdots\}$ that is, where the differential of counting process $A$, counting the transmission attempts and formally defined by 
%\[A(t)=\sup\{l\geq0:\sum_{i=0}^l\tau_i<t\},\] where $\tau_i=\sigma_i-\sigma_{i-1}$, is positive. However, in general, the reward function $r(t)$ allows to capture continuous cost, e.g. energy cost which can be proportional to the buffer occupancy at time $t$. Note that $r_m$ may be equivalent to a size of the successfully decoded packet transmitted in transmission opportunity $m$, or to a constant reward $r_m=C$, regardless of its size; it may incorporate additional cost factors predefined by DM. Without loss of generality, we assume that lost or dropped packets yield no reward. 
%\else
%The performance criterion is the expected total discounted infinite horizon reward which is given by the following well-known definition %\iflong
Consider an SMDP with discounted cost functional, characterized  by the tuple \sdo{\{\bS,\bA,\bP,r, \gamma\}}, where the components stand for the state space, the action space, the transition probabilities, the reward function and  the discount factor. The state space expresses the set of all possible combinations of buffer state, channel state, and leading packet size. The action space is a set of actions which fits exactly one action to one operating point. The state transitions probability space is calculated according to the transmission, arrival times distribution and channel and packet size dynamics. The reward is a symbolic representation of the accumulated throughput and, finally,  $\gamma$ is an appropriately selected constant.

Denote the ending time of $m$-th transmission attempt as $\sigma_m$, $m\in\{0,1,\cdots\}$. Clearly, positive rewards can be only added up at $\sigma_m$. The rewards, $r_m$ are r.v's, with expected value calculated in correspondence with some given policy $\pi$. Namely, in the case the transmission at time $\sigma_m$, according to selected action is successful, the reward was positive. In all other cases, $r_m$ is equal to zero.
Define $J^\pi(s_0)=\E\sum_{m=0}^\infty e^{-\gamma\sigma_{m}} r_m$.
In order to apply the dynamic programming principle, we view states right after a transmission starts. Define the augmented time series $\eta_m$, $m\in\{0,1,\cdots\}$, such that in the case a transmission is initiated at a non-empty system, the average discounted reward given by $\E r_me^{-\gamma\eta_{m}}$ is awarded. Hence, in the case a transmission starts right after arrival to the empty buffer, $r_m=0$, at $\eta_m$.

Write the discounted cost as the sum of reward obtained for the first transmission and average discounted residual throughput profit associated with future rewards. 
%
%\small
\begin{comment}
\req{-5}
{J^\pi(s_0)=\E\sum_{m=0}^\infty e^{-\gamma\sigma_{m}} r_m =\E r_0^\pi(s_0)+\E\sum_{m=1}^\infty e^{-\gamma\sigma_{m}} r_m}
{eq:disc}
\normalsize
\end{comment}
\begin{align}
& J^\pi(s_0) =\E r^\pi(s_0)e^{-\gamma\eta_{0}}+\E\sum_{m=1}^\infty e^{-\gamma\eta_{m}} r_m  \nonumber \\
& =\E r^\pi(s_0)+J^{\pi}_1(s_0)  \label{eq:disc}
\end{align}% \end{align}

Thus, our goal is the following:

Find the \textit{dynamic physical layer setting selection policy $\pi$}, which takes as input the current occupancy of the buffer and information (if any) on the current state of the channel and the packet size at the source's queue head, and provide as an output a decision on which transmission path to employ, such that $J^\pi(s_0)$ is maximized.  

Note that the analysis that follows can be easily extended to account for an average cost criteria, defined by 
 
$J^A=\lim_{N\to\infty}\frac{1}{N}\E\sum_{m=1}^N  r_m$ in the sense that both criteria possess  \textit{similar optimal policies}. 
The connection between discounted and average infinite reward criteria is understood via Blackwell optimality as it is demonstrated in e.g.,~\cite{bertsekas1995dynamic}.
%In particular, under mild conditions on $\gamma$, they  referred to as Blackwell optimal~\cite{bertsekas1995dynamic}.

 %Hence, average reward for action $u$ is given by $C(1-p_u)$. 
%Define average reward over infinite horizon
%In this paper, we only allow lump rewards at ending times of successful transmission attempts, denoted by $\sigma_m$, $m\in\{0,1,\cdots\}$.  We assumed a constant reward $r_m=C$, regardless of a packet size, however our model covers any lump reward function.

%\rals{-9}{
%J=&\E\int_0^\infty e^{-\gamma t} r(t)dt=\E\sum_{m=0}^\infty e^{-\gamma\sigma_m} r_m}	%\fi
%J^A=&\lim_{N\to\infty}\frac{1}{N}\E\sum_{m=1}^N  r_m} %=\E\sum_{m=0}^\infty e^{-\gamma\sigma_m} r_m}
%\iflong\else\normalsize\fi
%where $\gamma$ is a discount factor and $r(t)$ is a reward accumulated at time $t$.  %it may incorporate additional cost factors predefined by DM. Without loss of generality, we assume that lost or dropped packets yield no reward. 
%\fi%\iflong The second inequality merely solves the integral.\fi %Note that the expected value is over the interval boundaries as. 


Hence, we formulate the described problem by a discounted SMDP, which is formally explained in the next section.


\begin{table}[h!]
\center
\begin{tabular}{l|l}
\hline
variable & description \\
\hline
% $\bS$ & state space of SMDP  \\
% $\bA$ & action space \\
% $\calU $ & policy space  \\
                $\lambda$ & arrival rate \\
$\BS$ & buffer capacity (including the packet being transmitted) \\\hdashline
% $N$ & random variable characterizing number  of packets in  & $N \in \{0,1,\ldots,B-1 \}$  \\
% & queue, i.e.,  waiting queue + under transmission & \\ 
%             & (as states are tracked  right after  a service & \\ 
%          &   completes, $N \leq B-1$) & \\   
$s$ & SMDP state (buffer state,channel state,leading packet size) \\
%& Note: as state transitions occur after departures, the buffer \\
% & state after a transition  ranges between 0 and $B-1$ \\      
   $V(s)$ &   value function at state $s$, $V(s)=\max\{V^{(r)}(s),V^{(d)}(s)\}$ \\
    $V^{(u)}(s)$ &   cost associated with decision $u$ at state $s$, $u \in \{ a,b\}$   \\
  %   $V^{(b)}(s)$ &  cost associated with decision ``b" at state $s$     \\   \hdashline
    %$c_r$ & instantaneous relay throughput (reward) & $(1-p_r)C\beta_r$ \\
     %   $c_d$ & instantaneous direct throughput (reward) & $(1-p_d)C\beta_d$ \\
        $\beta_{u,s}$ &  discount associated with action $u$ \\
        $k$ &  number of frames  per packet \\
                     $\tau_{u,s}$ & mean time to transmit via channel $u$ at state $s$ \\
       %  $\tau_{b,s}$ & mean time to transmit via channel ``b" at state $s$ \\
                $\mu_{u,s}$ & transmission rate of channel $u$,          $\tau_{u,s} = 1/\mu_{u,s}$ \\ \hdashline
       % $\mu_{b,s}$ & transmission rate of channel ``b",           $\tau_{b,s} = % 1/\mu_{b,s}$ \\ \hdashline
        $p_u$ & packet loss probability associated with channel $u$, $u \in \{a,b\}$ \\ 
  %      $p_b$ & packet loss probability associated with channel ``b"\\   \hdashline
%        $\gamma$ & discount factor \\ 
%        $\pi$ & policy (subscript) \\ \hdashline
        $g^{\pi}(t)$ & pdf of transmission time then using policy $\pi$ \\ 
        $P^u(j|i,t)$ & probability of $j-i$ arrivals after $t$ time units, given a \\
        & buffer initially filled with $i$ packets and action  $u$  is taken  \\
        $p(h'|h)$ & channel transition probabilities \\
        $q(k'|k)$ & packet size transition probabilities\\%, given  action  $u$ is taken \\
       \hline
\end{tabular}
\vspace{-2pt}
\caption{SMDP notation.} \vspace{-0.25in} %\label{tab:general}
\end{table}


==> phy_model_O.tex <==
\begin{figure}
	\center
	\includegraphics[scale=0.29]{3to2}
	\vspace*{-5pt}\caption{Relay channel logical model}\label{fig:32} \vspace*{-15pt}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{System model and metrics}{\label{sec:phy}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The goal of this paper is to introduce a novel decision process approach that takes decisions and actions based on the current system state and parameters such as channel state, bit error rate, buffer occupancy, etc. In this section, we introduce the model that is used throughout the paper. In particular, we address both communication related and decision process related aspects.

\subsubsection*{\textbf{Arrival process}}
We assume a source (S) transmitting data to a destination (D). We assume that the data at the source are generated according to a Poisson process with intensity $\lambda$. \off{Note that the source and destination are not necessarily the origin or the final destination of the data, i.e., the data can be generated in previous entities and just need to be forwarded by the source to the next hop or can be generated by the source’s Application layer and be forwarded to the next hop.} We assume that pending packets waiting for transmission are stored in a finite size buffer which can occupy at most $B$ packets. The packets arriving at a full buffer are rejected and the retransmission details are taken care of by higher layers. Note that the number of packets that can be stored is limited to $B$ packets regardless of actual size. Such a model can describe a setup in which the packets’ descriptors are stored in the buffer whereas the varied size packets themselves are stored elsewhere. An extension which considers packets with varying buffer occupancy and specifically ones which occupy a varying number of \textit{chunks} in the buffer is addressed in~\ref{subsubsec1}.

\subsubsection*{\textbf{Transmission modes (action space)}}
The source attempts to communicate the packet at the head of the queue to the destination by choosing among the possible \textit{operating points} of the physical layer. Specifically, prior to each packet transmission, the DM needs to determine which Physical layer configuration to utilize for the next transmission. These ``options” constitute the DM action space. For example, in the relay network model the DM needs to determine whether to utilize the relay or to send the data directly to the receiver, or whether to use Amplify-and-Forward or Decode-and-Forward scheme for its next transmission. We will assume that each configuration has some advantage over the other configurations by at least one performance criteria. Accordingly, the DM needs to decide on the next action given the system state.

Throughout this paper we will assume only two possible operating points at all decision epochs. For ease of presentation and with no loss of generality, throughout this paper we will adopt the diversity-multiplexing tradeoff terminology from the classic half-duplex relay channel choice, and assume that one configuration is more reliable (i.e., lower bit error rate (BER)) at the expense of lower transmission rate, while the other configuration is less reliable (higher BER) yet provides higher transmission rate. Henceforth, we denote the more reliable configuration with a lower rate by ``a”, while the less reliable path with a higher rate will be denoted by ``b". The rates will be denoted by $R_a$ and $R_b$, where $R_a<R_b$, and the corresponding packet loss probabilities by $p_a$ and $p_b$, where $p_a<p_b$, for configurations ``a” and ``b”, respectively. It is important to note that even though throughout most of this paper we assume a simplified model in which each configuration is characterized by a fixed transmission rate and BER (i.e., the tuples $p_a, R_a$ and $p_b, R_b$ are fixed at all times) our model supports a straightforward extension in which the transmission rate and the BER on each operating point can vary depending on an underlay varying channel model. In Section~\ref{} we provide such an example, in which the channel at each operation point can experience two conditions associated with Good or Bad channel, which are modeled according to the Gilbert-Elliot model.

\off{For tractability, throughout this paper we will assume only two possible operating points at all decision epochs. Specifically, we assume that the sender can either send the next packet in configuration $a$ or in configuration $b$. We will assume that each configuration has some advantage over the other configurations by at least one performance criteria. For ease of presentation and with no loss of generality, throughout this paper we will adopt the diversity-multiplexing tradeoff terminology from the classic half-duplex relay channel choice, and assume that one configuration is more reliable (i.e., lower bit error rate (BER)) on the expense of lower transmission rate, while the other configuration is less reliable (higher BER) yet provides higher transmission rate. Henceforth, we associate the more reliable configuration with a lower rate with configuration ``a", while the less reliable path with a higher rate will be associated with configuration ``b". Denote the rates $R_a$ and $R_b$, where $R_a<R_b$. The corresponding packet loss probabilities are denoted as $p_a$ and $p_b$, where $p_a<p_b$ at all times. It is important to note that even though throughout most of this paper we assume a simplified model in which each configuration is characterized by a fixed transmission rate and BER (i.e., the tuples $p_a, R_a$ and $p_b, R_b$ are fixed) our model supports an extension in which the transmission rate and the BER on each operating point can varied relying on an underlay channel model. In Section~\ref{} we provide such an example, in which the channel on each operation point can experience two conditions associated with Good or Bad channel 'which are modeled according to the Gilbert-Elliot model. }

\FMO{This discussion should be moved to the section which introduces the Gilbert-Elliot model*** The reader should further note that allowing an underlying  channel model which can change over time raises an additional operating point in which the transmitter delays its transmission waiting for the channel to improve. For the sake of simplicity of presentation, we omit such operating point from this paper. Yet, the extension to include the option or not to transmit for the certain time period is technically tractable; the interested reader is referred to the online version of the paper for detail.}

We would like to emphasize that the restriction to only two configurations is only for tractability (presentation and analytical simplicity), and the extension to more than two possible operating points, or to different performance criteria as might be appropriate for other PHY layer configurations or other models, is straightforward.

\subsubsection*{\textbf{Transmission time (service model)}}
We consider packets of random length, hence, each operating point is characterized by a different service time which is modeled as a random variable with known distribution. We denote the transmission time probability density functions (pdf) $g^{a}(t)$ and $g^{b}(t)$, for configurations $a$ and $b$, respectively. Note that in the case of a half-duplex relay model example, $g^{a}(t)$ refers to the entire path associated with choice ``a", even though this configuration is subdivided into two separate paths (Figure~\ref{fig:32}).

We consider two modes: In the first mode, the packet size cannot be sampled by the DM in a timely fashion, hence is unknown prior to the transmission. In the second mode, the size of the upcoming packet is known to the DM prior to the transmission. Note that in both cases the fact that the DM has some knowledge (statistical or the actual size itself) regarding the next packets can influence its decision. We allow the packet size (hence transmission time) of a packet to be dependent on the previous packet size (transmission time). Specifically, we denote by $q(k'|k)$ the probability of having packet of size $k'$ at the head of the queue after transmitting packet of size $k$. We assume a finite set of possible packet sizes such that \rdo{\sum_{k'}q(k'|k)=1}. Note that $q$ can capture complex packet arrival patterns. For example, a sequence of big packets which is likely to be followed by a sequence of small packets and vice versa can be modeled provided the appropriate values for $q$ are selected. Obviously $q$ can omit any such correlation assuming that each packet is generated independently between packets, i.e., $q(k'|k)= q(k')$.


\subsubsection*{\textbf{Reward function}} We assume that the transmitter receives an instantaneous reward after each successfully transmitted packet. We denote by $r_m$ the reward attained by the transmitter after transmitting packet $m$. The reward can take multiple values taking into account many parameters such as packet size or transmission time. For simplicity throughout this paper we will assume a binary reward taking the value 1 for a successful transmission and 0 for an unsuccessful transmission ($r_m=0$ indicates that the packet was not received successfully by the receiver).

\subsubsection*{\textbf{General performance criterion}} A decision regarding which Physical layer configuration to select must be made prior to every transmission. A decision which affects the transmission duration and whether it was successful or not. Positive rewards are accumulated at the end of successful transmissions. In this paper we consider the infinite-horizon performance criterion for which the long-run accumulated reward is taken into account, yet the rewards that are received in the future are discounted according to how far away in time they will be received. Accordingly, we define a discount factor $\gamma \; (0\leq \gamma < 1)$, which captures the difference in importance between future rewards and present rewards. Note that in this discounted case, rewards obtained later are discounted more than rewards obtained earlier. Specifically, given the initial state $s_0$, the average discounted reward is given by:

\begin{equation}
\label{Eq_AverageDiscountedReward}
 J^\pi(s_0)=\E \sum_{m=0}^\infty r_m e^{-\gamma \sigma_m}
\end{equation}

\off{Thus, our goal is as follows: Find the \textit{dynamic physical layer setting selection policy $\pi$}, which takes as input the current occupancy of the buffer and information (if any) on the current state of the channel and the packet size at the source's queue head, and provide as an output a decision on which transmission path to employ, such that $J^\pi(s_0)$ is maximized.}

At each decision epoch (transmission opportunity) the DM needs to choose an action (Physical layer configuration for the next transmission) based on the system state (e.g., the buffer occupancy, the channel condition, the transmitted packet size, and any other prominent parameter). Note that the sojourn time and the system state until the next decision epoch depend only on the present state and the subsequently chosen action and are independent of past history of the system. Also, the reward attained depends only on the action chosen in that state. Accordingly, the DM objective is to determine a policy which optimizes the system performance (utility) described in (\ref{Eq_AverageDiscountedReward}), i.e., to determine an action to each transmission opportunity given the system state, which maximizes the infinite-horizon expected discounted reward. Note that the DM needs to balance short and long term reward considering that high short term reward can bring the system to inferior configuration for future rewards. For instance, choosing the lower transmission rate option when the buffer is almost full can result in packet loss due to buffer overflow. Alternatively, choosing the higher transmission rate when the buffer is completely or nearly empty and there is no urge to rush, risks the transmission to fail.

Note that the analysis that follows can be extended to account for an average cost criteria, defined by $J^A=\lim_{N\to\infty}\frac{1}{N}\E\sum_{m=1}^N  r_m$ in the sense that both criteria possess  \textit{similar optimal policies}. The connection between discounted and average infinite reward criteria is understood via Blackwell optimality as it is demonstrated in e.g.,~\cite{bertsekas1995dynamic}.


Hence, we formulate the described problem by a discounted SMDP, which is formally explained in the next section.


\begin{table}[h!]
\center
\begin{tabular}{l|l}
\hline
variable & description \\
\hline
% $\bS$ & state space of SMDP  \\
% $\bA$ & action space \\
% $\calU $ & policy space  \\
                $\lambda$ & arrival rate \\
$\BS$ & buffer capacity (including the packet being transmitted) \\\hdashline
% $N$ & random variable characterizing number  of packets in  & $N \in \{0,1,\ldots,B-1 \}$  \\
% & queue, i.e.,  waiting queue + under transmission & \\
%             & (as states are tracked  right after  a service & \\
%          &   completes, $N \leq B-1$) & \\
$s$ & SMDP state (buffer state,channel state,leading packet size) \\
%& Note: as state transitions occur after departures, the buffer \\
% & state after a transition  ranges between 0 and $B-1$ \\
   $V(s)$ &   value function at state $s$, $V(s)=\max\{V^{(r)}(s),V^{(d)}(s)\}$ \\
    $V^{(u)}(s)$ &   cost associated with decision $u$ at state $s$, $u \in \{ a,b\}$   \\
  %   $V^{(b)}(s)$ &  cost associated with decision ``b" at state $s$     \\   \hdashline
    %$c_r$ & instantaneous relay throughput (reward) & $(1-p_r)C\beta_r$ \\
     %   $c_d$ & instantaneous direct throughput (reward) & $(1-p_d)C\beta_d$ \\
        $\beta_{u,s}$ &  discount associated with action $u$ \\
        $k$ &  number of frames  per packet \\
                     $\tau_{u,s}$ & mean time to transmit via channel $u$ at state $s$ \\
       %  $\tau_{b,s}$ & mean time to transmit via channel ``b" at state $s$ \\
                $\mu_{u,s}$ & transmission rate of channel $u$,          $\tau_{u,s} = 1/\mu_{u,s}$ \\ \hdashline
       % $\mu_{b,s}$ & transmission rate of channel ``b",           $\tau_{b,s} = % 1/\mu_{b,s}$ \\ \hdashline
        $p_u$ & packet loss probability associated with channel $u$, $u \in \{a,b\}$ \\
  %      $p_b$ & packet loss probability associated with channel ``b"\\   \hdashline
%        $\gamma$ & discount factor \\
%        $\pi$ & policy (subscript) \\ \hdashline
        $g^{\pi}(t)$ & pdf of transmission time then using policy $\pi$ \\
        $P^u(j|i,t)$ & probability of $j-i$ arrivals after $t$ time units, given a \\
        & buffer initially filled with $i$ packets and action  $u$  is taken  \\
        $p(h'|h)$ & channel transition probabilities \\
        $q(k'|k)$ & packet size transition probabilities\\%, given  action  $u$ is taken \\
       \hline
\end{tabular}
\vspace{-2pt}
\caption{SMDP notation.} \vspace{-0.25in} %\label{tab:general}
\end{table}

